An enhanced decoding algorithm for coded compressed sensing

Coded compressed sensing is an algorithmic framework tailored to sparse recovery in very large dimensional spaces. This framework is originally envisioned for the unsourced multiple access channel, a wireless paradigm attuned to machine-type communications. Coded compressed sensing uses a divide-and-conquer approach to break the sparse recovery task into sub-components whose dimensions are amenable to conventional compressed sensing solvers. The recovered fragments are then stitched together using a low complexity decoder. This article introduces an enhanced decoding algorithm for coded compressed sensing where fragment recovery and the stitching process are executed in tandem, passing information between them. This novel scheme leads to gains in performance and a significant reduction in computational complexity. This algorithmic opportunity stems from the realization that the parity structure inherent to coded compressed sensing can be used to dynamically restrict the search space of the subsequent recovery algorithm.

==> TreeCodes/Bell_diagram.tex <==
\begin{tikzpicture}[
  font=\scriptsize, >=stealth', line width=1.25pt, line cap=round,
  node/.style={circle, minimum size=3.25mm, inner sep=0pt, draw=black}
]

\node[node] (s1) at (0,3.1) {1};
  \node[node] (s1-1) at (1,3.1) {1};
    \node[node] (s1-1-1) at (2.5,3.1) {1};
      \node[node,label=right:{$(1,1,1,1)$}] (s1-1-1-1) at (5,3.1) {1};
      \node[node,label=right:{$(1,1,1,4)$}] (s1-1-1-4) at (5,-1.5) {3};
    \node[node] (s1-1-3) at (2.5,-0.5) {3};
      \node[node,label=right:{$(1,1,3,1)$}] (s1-1-3-1) at (5,1.9) {3};
      \node[node,label=right:{$(1,1,3,3)$}] (s1-1-3-3) at (5,-0.5) {3};
      \node[node,label=right:{$(1,1,3,4)$}] (s1-1-3-4) at (5,-2.7) {6};
  \node[node] (s1-2) at (1,0.9) {3};
    \node[node] (s1-2-1) at (2.5,2.7) {3};
      \node[node,label=right:{$(1,2,1,1)$}] (s1-2-1-1) at (5,2.7) {3};
      \node[node,label=right:{$(1,2,1,2)$}] (s1-2-1-2) at (5,0.9) {3};
      \node[node,label=right:{$(1,2,1,4)$}] (s1-2-1-4) at (5,-1.9) {6};
    \node[node] (s1-2-2) at (2.5,0.9) {3};
      \node[node,label=right:{$(1,2,2,1)$}] (s1-2-2-1) at (5,2.3) {3};
      \node[node,label=right:{$(1,2,2,2)$}] (s1-2-2-2) at (5,0.5) {3};
      \node[node,label=right:{$(1,2,2,4)$}] (s1-2-2-4) at (5,-2.3) {6};
    \node[node] (s1-2-3) at (2.5,-0.9) {6};
      \node[node,label=right:{$(1,2,3,1)$}] (s1-2-3-1) at (5,1.5) {6};
      \node[node,label=right:{$(1,2,3,2)$}] (s1-2-3-2) at (5,0.1) {6};
      \node[node,label=right:{$(1,2,3,3)$}] (s1-2-3-3) at (5,-0.9) {6};
      \node[node,label=right:{$(1,2,3,4)$}] (s1-2-3-4) at (5,-3.1) {6};

\draw[line width=0.5pt] (s1) -- (s1-1);
  \draw[line width=0.5pt] (s1-1) -- (s1-1-1);
    \draw[line width=0.5pt] (s1-1-1) -- (s1-1-1-1);
    \draw[line width=1.5pt] (s1-1-1) -- (s1-1-1-4);
  \draw[line width=1.5pt] (s1-1) -- (s1-1-3);
    \draw[line width=1.5pt] (s1-1-3) -- (s1-1-3-1);
    \draw[line width=1.5pt] (s1-1-3) -- (s1-1-3-3);
    \draw[line width=3.0pt] (s1-1-3) -- (s1-1-3-4);
\draw[line width=1.5pt] (s1) -- (s1-2);
  \draw[line width=1.5pt] (s1-2) -- (s1-2-1);
    \draw[line width=1.5pt] (s1-2-1) -- (s1-2-1-1);
    \draw[line width=1.5pt] (s1-2-1) -- (s1-2-1-2);
    \draw[line width=3.0pt] (s1-2-1) -- (s1-2-1-4);
  \draw[line width=1.5pt] (s1-2) -- (s1-2-2);
    \draw[line width=1.5pt] (s1-2-2) -- (s1-2-2-1);
    \draw[line width=1.5pt] (s1-2-2) -- (s1-2-2-2);
    \draw[line width=3.0pt] (s1-2-2) -- (s1-2-2-4);
  \draw[line width=3.0pt] (s1-2) -- (s1-2-3);
    \draw[line width=3.0pt] (s1-2-3) -- (s1-2-3-1);
    \draw[line width=3.0pt] (s1-2-3) -- (s1-2-3-2);
    \draw[line width=3.0pt] (s1-2-3) -- (s1-2-3-3);
    \draw[line width=3.0pt] (s1-2-3) -- (s1-2-3-4);

\draw[dashed] (-0.4,3.4) -- (6.8,3.4);
\draw[dashed] (-0.1,1.2) -- (6.5,1.2);
\draw[dashed] (-0.1,-0.2) -- (6.5,-0.2);
\draw[dashed] (-0.1,-1.2) -- (6.5,-1.2);
\draw[dashed] (-0.4,-3.4) -- (6.8,-3.4);

\node[rotate=90] at (-0.4,2.3) {\small level~$0$};
\node[rotate=90] at (-0.4,0.5) {\small level~$1$};
\node[rotate=90] at (-0.4,-0.7) {\small level~$2$};
\node[rotate=90] at (-0.4,-2.3) {\small level~$3$};

\node[rotate=-90] at (6.8,0) {\small $j$-patterns $\sv$};
\end{tikzpicture}

==> TreeCodes/Bellnumbers.tex <==
\begin{tikzpicture}
[font=\normalsize, >=stealth', line width=1pt]

\node (v1) at (2.625,3) {${\genfrac..{0pt}{1}{1}{(1)}}$};
\node (v2) at (0.75,1.5) {${\genfrac..{0pt}{1}{1}{(1,1)}}$};
\node (v3) at (4.5,1.5) {${\genfrac..{0pt}{1}{K-1}{(1,2)}}$};
\node (v4) at (0,0) {${\genfrac..{0pt}{1}{1}{(1,1,1)}}$};
\node (v5) at (1.5,0) {${\genfrac..{0pt}{1}{K-1}{(1,1,3)}}$};
\node (v6) at (3,0) {${\genfrac..{0pt}{1}{K-1}{(1,2,1)}}$};
\node (v7) at (4.5,0) {${\genfrac..{0pt}{1}{K-1}{(1,2,2)}}$};
\node (v8) at (6,0) {${\genfrac..{0pt}{1}{(K-1)(K-2)}{(1,2,3)}}$};
\node (p1) at (-1.5, 3) {$\mathcal{P}_1:$};
\node (p2) at (-1.5, 1.5) {$\mathcal{P}_2:$};
\node (p3) at (-1.5, 0) {$\mathcal{P}_3:$};
\draw[->] (v1) edge (v2);
\draw[->] (v1) edge (v3);
\draw[->] (v2) edge (v4);
\draw[->] (v2) edge (v5);
\draw[->] (v3) edge (v6);
\draw[->] (v3) edge (v7);
\draw[->] (v3) edge (v8);

\end{tikzpicture}




==> TreeCodes/Full_plot_Bell_numbers.tex <==
\begin{tikzpicture}

\begin{axis}[%
font=\footnotesize,
width=7cm,
height=5.5cm,
scale only axis,
xmin=0,
xmax=10,
xtick = {0,1,...,10},
xlabel={\small Sub-Block Index $j$},
xmajorgrids,
ymin=1,
ymax=6,
ytick = {1,2,...,7},
ylabel={\small Expected Number of Surviving Paths},
ymajorgrids,
legend style={at={(0,1)},anchor=north west,draw=black,fill=white,legend cell align=left}
]

\addplot [color=cyan,dashed,line width=1.5pt]
  table[row sep=crcr]{
0 1.000\\
1 4.1094\\
2 4.2065\\
3 4.2825\\
4 4.3418\\
5 4.3881\\
6 4.4243\\
7 4.4526\\
8 4.4747\\
9  1.1091\\
10 1.0067\\
};
\addlegendentry{Approximation $\mathbb{E}[\tilde{L}_j]$};

\addplot [color=blue,solid,line width=1.5pt]
  table[row sep=crcr]{
0 1.000\\
1 4.1154\\
2 4.2234\\
3 4.3139\\
4 4.3908\\
5 4.4570\\
6 4.5150\\
7 4.5666\\
8 4.6132\\
9  1.1685\\
10 1.0695\\
};
\addlegendentry{Numerical $\mathbb{E}[L_j]$};

\addplot [color=black,dotted,line width=1.5pt]
  table[row sep=crcr]{
0 1.000\\
1 4.1146\\
2 4.2197\\
3 4.3105\\
4 4.3880\\
5 4.4559\\
6 4.5119\\
7 4.5656\\
8 4.6135\\
9  1.1689\\
10 1.0693\\
};
\addlegendentry{Simulated $\mathbb{E}[L_j]$};



\end{axis}

\end{tikzpicture}%

==> TreeCodes/subvector.tex <==
\begin{tikzpicture}[
  font=\small, >=stealth', line width=0.75pt,
  infobits/.style={rectangle, minimum height=7mm, minimum width=40mm, draw=black, fill=gray!10, rounded corners},
  paritybits/.style={rectangle, minimum height=7mm, minimum width=20mm, draw=black, fill=gray!40, rounded corners}
]

\node[infobits] (vb) at (2,0) {$\wv$};
\node[paritybits] (vp) at (5,0) {$\pv$};
\node (bits) at (-0.4,0) {$\vv$};
\draw[|-|] (0,-0.5) to node[midway,below] {$m$ bits} (4,-0.5);
\draw[-|] (4,-0.5) to node[midway,below] {$l$ bits} (6,-0.5);

\end{tikzpicture}



==> TreeCodes/subvectors3.tex <==
\begin{tikzpicture}[
  font=\small, >=stealth', line width=0.75pt,
  infobits/.style={rectangle, minimum height=7mm, minimum width=10mm, draw=black, fill=gray!10, rounded corners},
  paritybits/.style={rectangle, minimum height=7mm, minimum width=10mm, draw=black, fill=gray!40, rounded corners}
]

\node[infobits, minimum width=20mm] (vb0) at (1,0) {$\wv(0)$};
\node[infobits] (vb1) at (2.5,0) {$\wv(1)$};
\node[paritybits] (vp1) at (3.5,0) {$\pv(1)$};
\node[infobits] (vb2) at (4.5,0) {$\wv(2)$};
\node[paritybits] (vp2) at (5.5,0) {$\pv(2)$};
\node[infobits] (vb3) at (6.5,0) {$\wv(3)$};
\node[paritybits] (vp3) at (7.5,0) {$\pv(3)$};
\node (bits) at (-0.4,0) {$\vv$};
\draw[|-|] (0,-0.5) to node[midway,below] {$m_0$} (2,-0.5);
\draw[-|] (2,-0.5) to node[midway,below] {$m_1$} (3,-0.5);
\draw[-|] (3,-0.5) to node[midway,below] {$l_1$} (4,-0.5);
\draw[-|] (4,-0.5) to node[midway,below] {$m_2$} (5,-0.5);
\draw[-|] (5,-0.5) to node[midway,below] {$l_2$} (6,-0.5);
\draw[-|] (6,-0.5) to node[midway,below] {$m_3$} (7,-0.5);
\draw[-|] (7,-0.5) to node[midway,below] {$l_3$} (8,-0.5);

\end{tikzpicture}



==> TreeCodes/treecodes.tex <==
% \documentclass[journal,draftcls,onecolumn]{IEEEtran}
% \input{preamble}

% \begin{document}

\section{Performance of Tree Code}
\label{Section:PerformanceTreeCodeAppendix}

In this section, we characterize the performance of tree codes, as they pertain to coded compressive sensing.
To do so, we briefly review relevant results related to random linear codes.
We then extend these results to the desired setting.
As we will see shortly, the exact analysis of the probability of failure under tree decoding, although tractable, is cumbersome, especially for deep trees.
Nevertheless, a precise expression can be derived for performance characterization, and it is employed to compute probabilities of error for the parameters of interest.


\subsection{Random Linear Codes}
\label{sectionRandomLInearCodes}

To begin, we inspect the type of (random) linear codes we are interested in.
Consider a binary information vector $\wv$ of length $m$.
This vector is systematically encoded using parity generator matrix $G$ of size $m \times l$.
The resulting codeword, $\vv = \wv \pv$, is then obtained by taking message $\wv$ and appending parity vector $\pv$ to it.
Specifically, the parity bits are generated via linear equation
\begin{equation*}
\pv = \wv G ,
\end{equation*}
where operations are taken over binary field $\mathbb{F}_2$.
Thus, $\vv$ has length $m + l$, as depicted in Fig.~\ref{figure:subvector}.
\begin{figure}[htb]
  \centering
  \input{TreeCodes/subvector}
  \caption{Message $\vv$ is obtained through systematic encoding.
  It is composed of $m$ information bits and $l$ parity-check bits.}
  \label{figure:subvector}
\end{figure}

Suppose that an alternate information vector $\wv_{\mathrm{r}}$ is selected at random from $\{ 0, 1 \}^m$.
This vector is encoded using the same generator matrix $G$, yielding concatenated vector $\vv_{\mathrm{r}} = \wv_{\mathrm{r}} \pv_{\mathrm{r}}$ with $\pv_{\mathrm{r}} = \wv_{\mathrm{r}} G$.
We wish to compute the probability that $\vv$ and $\vv_{\mathrm{r}}$ share a same parity sub-component, i.e., $\pv = \pv_{\mathrm{r}}$.

\begin{lemma}
Fix information vector $\wv$ and parity generating matrix $G$.
The probability that a randomly selected information vector $\wv_{\mathrm{r}} \in \{ 0, 1 \}^m$ produces the same parity sub-component as $\wv$ under $G$ is given by
\begin{equation*}
\Pr (\pv = \pv_{\mathrm{r}}) = 2^{- \operatorname{rank} (G)} .
\end{equation*}
\end{lemma}
\begin{IEEEproof}
Information vector $\wv_{\mathrm{r}}$ is drawn at random, uniformly over $\{ 0, 1 \}^m$.
Codeword $\vv_{\mathrm{r}}$ is then created by computing parity bits $\pv_{\mathrm{r}} = \wv_{\mathrm{r}} G$ and, subsequently, appending these bits to the information vector.
This process yields codeword $\vv_{\mathrm{r}} = \wv_{\mathrm{r}} \pv_{\mathrm{r}}$.
The event $\{ \pv = \pv_{\mathrm{r}} \}$ can therefore be expressed as
\begin{equation*}
\begin{split}
\{ \pv = \pv_{\mathrm{r}} \}
&= \{ \wv G = \wv_{\mathrm{r}} G \}
= \{ (\wv + \wv_{\mathrm{r}}) G = \underline{0} \} \\
&= \{ \wv + \wv_{\mathrm{r}} \in \operatorname{nullspace}(G) \} .
\end{split}
\end{equation*}
Note that subtraction and addition are equivalent under operations in $\mathbb{F}_2$.
Moreover, vector $\wv + \wv_{\mathrm{r}}$ is uniformly distributed over $\{ 0, 1 \}^m$.
Since the number of vectors in the nullspace of $G$ is
$2^{\operatorname{nullity}(G)} = 2^{m - \operatorname{rank} (G)}$,
it follows that
\begin{equation*}
\Pr ( \pv = \pv_{\mathrm{r}} )
= \frac{2^{m - \operatorname{rank} (G)}}{2^m}
= \frac{1}{2^{\operatorname{rank}(G)}} .
\end{equation*}
This completes the proof.
\end{IEEEproof}

The rank of parity generator matrix $G$ is of fundamental importance in assessing performance.
In many scenarios, including our current treatment of unsourced multiple access, matrix $G$ is drawn at random from a large ensemble.
In such cases, it becomes appropriate to compute the probability that an erroneous vector fulfills the parity constraints associated with $\wv$.

\begin{lemma} \label{lemma:RandomGenerator}
Fix erroneous vector $\wv_{\mathrm{e}} \neq \wv$.
Let parity generator matrix $G$ be a Rademacher matrix of size $m \times l$.
That is, the entries in $G$ are drawn at random from a uniform Bernoulli distribution, independently of one another.
Under such circumstances, the probability of event $\{ \pv = \pv_{\mathrm{e}} \}$ is given by
\begin{equation*}
\Pr (\pv = \pv_{\mathrm{e}}) = 2^{-l} .
\end{equation*}
\end{lemma}
\begin{IEEEproof}
The event $\{ \pv = \pv_{\mathrm{e}} \}$ is equivalent to $\{ (\wv + \wv_{\mathrm{e}})G = \underline{0} \}$.
Since $\wv \neq \wv_{\mathrm{e}}$, there exists at least one pair of vector entries, say at location~$q$, such that $\wv(q) + \wv_{\mathrm{e}}(q) = 1$.
Then,
\begin{equation*}
(\wv + \wv_{\mathrm{e}})G
= G[q,:] + \sum_{\ell \neq q} (\wv(\ell) + \wv_{\mathrm{e}}(\ell))G[\ell,:] ,
\end{equation*}
where $G[q,:]$ denotes the $q$th row of $G$.
By constructions, $G[q,:]$ is a sequence of independent, uniform Bernoulli trials.
Therefore, $(\wv + \wv_{\mathrm{e}})G$ also forms a sequence of independent, uniform Bernoulli bits and, hence, the probability that this sequence is the all-zero sequence is equal to $2^{-l}$.
\end{IEEEproof}

Conceptually, the results presented in this section form the cornerstones of our upcoming analysis.
However, when codewords are fragmented and redundancy is added at different stages, assessing performance becomes more complicated.
We initiate our treatment of this more elaborate scenario next.


\subsection{Fragmented Codewords}
\label{subsection:FragmentedCodewrds}

An important distinction that arises in coded compressive sensing when compared to standard random linear codes stems from the fragmented structure of tree codes depicted in Fig.~\ref{figure:subvector3}.
A second related factor ensues from the fact that erroneous candidates are formed by piecing together fragments from valid codewords.
Typically, when studying error events under random linear coding, the starting point is an erroneous message of the form $\wv_{\mathrm{e}} \neq \wv$, as in Lemma~\ref{lemma:RandomGenerator}.
However, the situation is more intricate for tree coding and meticulous accounting must be performed.
\begin{figure}[htb]
  \centering
  \input{TreeCodes/subvectors3}
  \caption{The fragmented nature of tree coding leads to peculiarities in the performance analysis of this scheme.
  This situation arises, partly, from the fact that two different information sequences can share identical fragments.}
  \label{figure:subvector3}
\end{figure}

There are essentially three confounding factors in the analysis of erroneous messages in tree coding.
First, several fragments within an erroneous candidate codeword may come from a same message.
Such occurrences can significantly reduce the discriminating power of parity bits.
Second, two different messages may have overlapping information fragments, as they only need to differ at one location overall.
Thence, when comparing a valid codeword to an erroneous candidate, the two messages are necessarily distinct, yet some of their information fragments may be identical.
Third, the loss of discriminating power from parity bits is correlated across fragments in certain cases, which exacerbates the probability of detection failure.
We elaborate on these idiosyncrasies below.

Suppose $\wv = \wv(0) \wv(1) \cdots \wv(n-1)$ is a partitioned information vector.
Let
\begin{equation} \label{equation:CodewordStructure}
\vv = \wv(0) \wv(1) \pv(1) \cdots \wv(n-1) \pv(n-1)
\end{equation}
be the corresponding codeword produced by tree encoding.
Since parity bits only operate on information bits contained in fragments that precede a slot, the generator matrix admits an upper triangular block structure of the form
\begin{equation*}
G = \begin{bmatrix} G_{0,0} & G_{0,1} & G_{0,2} & \cdots \\
\mathbf{0} & G_{1,1} & G_{1,2} & \cdots \\
\mathbf{0} & \mathbf{0} & G_{2,2} & \cdots \\
\vdots & \vdots & \vdots & \ddots \end{bmatrix} .
\end{equation*}
The parity bits $\pv(j)$ are then produced by column group~$j$,
\begin{equation*}
\pv(j) = \sum_{\ell=0}^{j-1} \wv(\ell) G_{\ell,j-1} .
\end{equation*}
These parity bits are subsequently injected into the codeword as in \eqref{equation:CodewordStructure}.
We wish to capture the performance of the tree code when active blocks within $G$ are Rademacher sub-matrices.
That is, the entries of every sub-matrices are uniform Bernoulli trials, independent of one another and across blocks.

To examine the behavior of the tree code, consider a collection of codewords $\mathcal{L} = \{ \vv_1, \vv_2, \ldots, \vv_K \}$.
Under tree coding, every codeword has the form
\begin{equation*}
\vv_i = \wv_i(0) \wv_i(1) \pv_i(1) \cdots \wv_i(n-1) \pv_i(n-1)
\end{equation*}
where $\pv_i(j) = \sum_{\ell=0}^{j-1} \wv_i(\ell) G_{\ell,j-1}$.
The collection of fragment candidates at stage~$0$ is
\begin{equation*}
\mathcal{L}_0 = \{ \wv_i (0) : i = 1, \ldots, K \} .
\end{equation*}
Similarly, the list of fragment candidates at stage~$j$, where $j \in [1:n-1]$, can be expressed as
\begin{equation*}
\mathcal{L}_j = \{ \wv_i (j) \pv_i (j) : i = 1, \ldots, K \} .
\end{equation*}
The goal of the tree decoder is to produce an unordered list that matches the original set of messages $\mathcal{M} = \{ \wv_1, \wv_2, \ldots, \wv_K \}$.
We emphasize that valid messages invariably appear on the final output list because they necessarily fulfill their own parity constraints.
The probability of error is then dictated by instances where invalid codewords also meet their own parity constraints.
In such cases, the decoder fails to identify these extraneous candidates as erroneous and, therefore, they make it to the final output list as well.
As mentioned above, one of the challenges in analyzing error events is the fact that distinct candidate codewords are not guaranteed to have different fragments at any particular stage.
That is, information fragments can appear more than once in $\mathcal{M}_j = \{ \wv_1(j), \wv_2(j), \ldots, \wv_K(j) \}$, possibly paired with different parity bits.
This situation precludes the naive application of Lemma~\ref{lemma:RandomGenerator} in a divide-and-conquer fashion.

Consider the situation where the tree decoder seeks to validate codewords that start with root fragment $\wv_{i_0}(0)$.
For a given collection $\mathcal{L}$ of transmitted codewords, the list of candidate codewords visited during this portion of the tree decoding process is composed of elements of the form
\begin{equation} \label{equation:CandidateCodewords}
\begin{split}
&\vv_{\mathrm{c}} = \vv_{i_0}(0) \vv_{i_1}(1) \vv_{i_2} (2) \cdots \vv_{i_{n-1}}(n-1) \\
&= \wv_{i_0}(0) \wv_{i_1}(1) \pv_{i_1}(1) \cdots \wv_{i_{n-1}}(n-1) \pv_{i_{n-1}}(n-1) ,
\end{split}
\end{equation}
where $i_j \in [1:K]$ for all slots $j \in [1:n-1]$.
The ability of the tree code to discriminate between valid and erroneous sequences hinges on the structure of the candidate vectors in \eqref{equation:CandidateCodewords} and their connection to parity generator matrix $G$.
We turn our attention to the role of $G$ in identifying invalid codewords.

To survive stage~1, candidate vector $\vv_{\mathrm{c}}$ must fulfill $\pv_{i_1}(1) = \wv_{i_1}(0) G_{0,0} = \wv_{i_0}(0) G_{0,0}$.
Equivalently, we can write $(\wv_{i_0}(0) + \wv_{i_1}(0)) G_{0,0} = \underline{0}$.
To outlast the first two stages, a candidate vector must fulfill two conditions,
\begin{gather*}
\pv_{i_1}(1) = \wv_{i_1}(0) G_{0,0} = \wv_{i_0}(0) G_{0,0} \\
\begin{split}
\pv_{i_2}(2) &= \left( \wv_{i_2}(0), \wv_{i_2}(1) \right)
\begin{bmatrix} G_{0,1} \\ G_{1,1} \end{bmatrix} \\
&= \left( \wv_{i_0}(0), \wv_{i_1}(1) \right)
\begin{bmatrix} G_{0,1} \\ G_{1,1} \end{bmatrix} .
\end{split}
\end{gather*}
This translates into linear equations
\begin{gather*}
\left( \wv_{i_0}(0) + \wv_{i_1}(0) \right) G_{0,0} = \underline{0} \\
\left( \wv_{i_0}(0) + \wv_{i_2}(0), \wv_{i_1}(1) + \wv_{i_2}(1) \right)
\begin{bmatrix} G_{0,1} \\ G_{1,1} \end{bmatrix}
= \underline{0} .
\end{gather*}
% Likewise, to withstand the first three stages, the same candidate codeword must meet conditions
% \begin{align*}
% \left( \wv_{i_0}(0) + \wv_{i_1}(0) \right) G_{0,0} &= \underline{0} \\
% \left( \wv_{i_0}(0) + \wv_{i_2}(0), \wv_{i_1}(1) + \wv_{i_2}(1) \right)
% \begin{bmatrix} G_{0,1} \\ G_{1,1} \end{bmatrix}
% &= \underline{0} \\
% \left( \wv_{i_0}(0) + \wv_{i_3}(0), \wv_{i_1}(1) + \wv_{i_3}(1), \wv_{i_2}(2) + \wv_{i_3}(2) \right)
% \begin{bmatrix} G_{0,2} \\ G_{1,2} \\ G_{2,2} \end{bmatrix}
% &= \underline{0} .
% \end{align*}
In general, to survive the first $j$ stages, a candidate vector must meet the constraints
\begin{equation} \label{equation:GeneralG}
\sum_{\ell = 0}^{q-1} \left( \wv_{i_{\ell}}(\ell) + \wv_{i_q}(\ell) \right) G_{\ell,q-1}
= \underline{0}
\end{equation}
for $q = 1, \ldots, j$.
Keeping these requirements in mind and factoring in the randomness in the problem, we can characterize the probability that an arbitrary candidate vector $\vv_{\mathrm{c}}$ survives the first $j$ stages by analyzing the number of nontrivial random linear equations it must satisfy.
In addressing this question, it is meaningful to study the effective number of parity constraints this candidate sequence must fulfill on a per slot basis.
The insight afforded by Lemma~\ref{lemma:RandomGenerator} is that the $l_j$ parity bits associated with stage~$j$ either act as a statistically discriminating sequence of independent Bernoulli samples, each with probability half, or they are fulfilled trivially based on the combined vector in \eqref{equation:GeneralG} vanishing.
More specifically, the criterion for the former condition to apply is that at least one of the entries in
\begin{equation} \label{equation:InputVector}
\left( \wv_{i_{0}}(0) + \wv_{i_j}(0), \ldots, \wv_{i_{j-1}}(j-1) + \wv_{i_j}(j-1) \right)
\end{equation}
is not equal to zero.
As mentioned above, there are two distinct phenomena that can drive individual entries in \eqref{equation:InputVector} to zero.
Matching occurs in a block fashion whenever $i_{\ell} = i_{j}$ for some $\ell < j$.
Under such circumstances, multiple portions of the candidate vector comes from valid codeword $\wv_{i_j}$ itself and, consequently, $\wv_{i_{\ell}}$ and $\wv_{i_j}$ match at the corresponding locations.
The second possibility arises from two distinct valid messages randomly sharing a common section.
At stage~$j$, the probability that two independent sub-blocks match one another is given by
\begin{equation*}
\Pr \left( \wv_{i_{\ell}}(\ell) = \wv_{i_j}(\ell) | i_{\ell} \neq i_j \right) = 2^{-m_{\ell}} ,
\end{equation*}
where $\ell \in \{ 0, \ldots, j-1 \}$.
Not surprisingly, this probability is intrinsically linked to the number of information bits contained in the sub-block.
We already know from Lemma~\ref{lemma:RandomGenerator} that there is a dichotomy between parity bits associated with column group~$j$.
A collection $\pv(j)$ of parity bits is either statistically discriminating or, as a block, it becomes uninformative.
The distinction between these two situations stems from the character of the input vectors in \eqref{equation:InputVector}, whether they are identical or different.
One subtlety related to the number of active parity bits for a particular candidate codeword can be seen by stacking the combined vectors,
\begin{gather*}
\left( \wv_{i_0}(0) + \wv_{i_1}(0) \right) \\
\left( \wv_{i_0}(0) + \wv_{i_2}(0), \wv_{i_1}(1) + \wv_{i_2}(1) \right) \\
% \left( \wv_{i_0}(0) + \wv_{i_3}(0), \ldots, \wv_{i_2}(2) + \wv_{i_3}(2) \right) \\
\vdots \\
\left( \wv_{i_0}(0) + \wv_{i_j}(0), \ldots, \wv_{i_{j-1}}(j-1) + \wv_{i_j}(j-1) \right) .
\end{gather*}
Whenever a candidate codeword draws multiple fragments from a same valid message, the events where the combined vectors vanish and the corresponding parity bits lose their discriminatory power become more likely within a block.
These events are also correlated across blocks.
For example, if $i_2 = i_3$ and $\wv_{i_0}(0) + \wv_{i_2}(0) = \underline{0}$, then $\wv_{i_0}(0) + \wv_{i_3}(0) = \underline{0}$.
Consequently, for certain index patterns, the probability that an erroneous candidate meets its parity constraints at different stages cannot be treated separately.
Altogether, the probability that candidate codeword $\vv_{\mathrm{c}}$ is consistent with its own parity bits depends on its index sequence, which can be taken as visits to distinct levels over the progression of the candidate message.

Let index sequence $i_0, i_1, \ldots, i_{n-1}$ be given.
We are interested in conditional probabilities of the form
\begin{equation*}
\Pr (T = t | i_0, i_1, \ldots, i_{n-1})
\end{equation*}
where $T$ is the number of statistically discriminating parity bits.
Since $i_j \in [1:K]$, there are $K^n$ possible conditions.
A careful examination of the problem and, in particular, of \eqref{equation:GeneralG} reveals that this probability is permutation invariant.
That is, the state labeling is irrelevant, only the order in which previously visited states are reentered matters.
Mathematically, the structure of the problem enables us to write
\begin{equation*}
\Pr (T = t | i_0, i_1, \ldots, i_{n-1})
= \Pr (T = t | \pi(i_0), \pi(i_1), \ldots, \pi(i_{n-1}))
\end{equation*}
for any permutation $\pi$ of the integers $1, \ldots, K$.
When the number of active devices exceeds the slot count, this symmetric property reduces the number of possible cases from $K^n$ to the $n$th Bell number (OEIS A000110) given by the formula
\begin{equation*}
B_n=\sum_{j=0}^n S_n^{(j)} .
\end{equation*}
Above, $S_n^{(j)}$ represents the Stirling numbers of the second kind (OEIS A008277), which can be computed recursively using the formula $S_n^{(j)} = S_{n-1}^{(j-1)} + j S_{n-1}^{(j)}$.


\subsection{Pattern Sequences}
\label{subsection:PatternSequence}

To simplify the problem and reduce the total number of cases to be considered, we leverage equivalence classes of erroneous patterns wherein every sequence within a class share the same probability of going undetected.
The structure of the equivalence classes is informed by $j$-patterns (OEIS A008277).
For completeness, we include an appropriate definition below.

\begin{definition}[$j$-Pattern Sequences] \label{definition:jPattern}
A $j$-pattern sequence is an integer sequence
\begin{equation*}
\sv = (\sv(0), \sv(1), \ldots, \sv(j-1))
\end{equation*}
such that $\sv(\ell) = \ell+1$ or $\sv(\ell) = \sv(q)$ for some $q \in [0:\ell-1]$.
\end{definition}

We denote the collection of all $j$-pattern sequences by $\mathcal{P}_j$, where $1 \leq j \leq n$.
There is a single $1$-pattern sequence, $\mathcal{P}_1 = \{ (1) \}$.
Similarly,
\begin{gather*}
\mathcal{P}_2 = \{(1,1), (1,2)\} \\
\mathcal{P}_3 = \{ (1,1,1), (1,1,3), (1,2,1), (1,2,2), (1,2,3) \}
\end{gather*}
indicate the collection of all $2$-pattern and $3$-pattern sequences, respectively.
To be consistent with our established notation, we index the entries of $j$-pattern sequence $\sv$ using integers $[0:j-1]$.
We  emphasize that a $j$-pattern sequence can be created iteratively starting with a shorter $(j-1)$-pattern sequence $\sv$ and appending to it either integer $j$ or entry $\sv(k)$ for some $k < j-1$.
With this construction, it can be verified that the total number of $j$-pattern sequences equal to the $j$th Bell number (OEIS A000110); that is, $|\mathcal{P}_j| = B_j$.

Under this viewpoint, each $j$-pattern sequence $\sv \in \mc{P}_j$ acts as a representative element to a collection of vectors of the form $(i_0, i_1, \ldots, i_{j-1})$.
The mapping from an arbitrary integer sequences in $[1:K]^n$ to the representative of its equivalence class can be defined recursively.
The initial entry of the representative is $\sv(0) = 1$, irrespective of $i_0$.
Then, for any $q > 1$,
\begin{equation*}
\sv(q) = \begin{cases} q+1 & i_{q} \notin \{ i_0, \ldots, i_{q-1} \} \\
\min  \{ \ell \in [1:q-1] \mid i_{\ell} = i_q \} & \text{otherwise} . \end{cases}
\end{equation*}
For instance, any vector of the form $\{(i_0,i_1,i_2):i_0=i_1=i_2\}$ maps to the $3$-pattern sequence $(1,1,1)$.
Likewise, any vector in $\{(i_0,i_1,i_2):i_0=i_1,i_1 \neq i_2\}$ map to $(1,1,3)$.
The number of admissible integer sequences within an equivalence class is characterized below.
Without loss of generality, we focus on a single rooted tree with $i_0 = 1$ to simplify our upcoming discussion.

\begin{lemma}\label{Number of states}
Let $\sv \in \mc{P}_j$ denote a $j$-pattern sequence.
The number of integer sequences $i_0, \ldots, i_{j-1}$ that map to $\sv$ is given by
\begin{equation} \label{equation:SizeEquivalenceClass}
n(\sv) = (K-1)(K-2) \cdots (K-(d(\sv)-1)),
\end{equation}
where $d(\sv)$ denotes the number of distinct integers in $\sv$.
\end{lemma}
\begin{IEEEproof}
By assumption, we have $i_0 = 1$.
For $\ell > 0$, integer $i_{\ell}$ is unambiguously determined by its predecessors whenever a previous entry is repeated in sequence $\sv$.
On the other hand, when $s(\ell) = \ell + 1$, integer $i_{\ell}$ can be any element within $[1:K]$ that has not appeared in the sequence thus far.
Combining these observations with a straightforward application of the counting principle, we get \eqref{equation:SizeEquivalenceClass}.
\end{IEEEproof}
The total number of candidate paths in the tree at stage $j-1$ is $\sum_{\sv \in \mc{P}_j}n(\sv)=K^{j-1}$.
Figure~\ref{figure:Bellnumbers} shows $j$-pattern sequences and the cardinality of their equivalence classes for stages $0$, $1$, and $2$ in the tree.
\begin{figure}[htb]
  \centering
  \input{TreeCodes/Bellnumbers}
  \caption{This illustration showcases $j$-pattern sequences for stages $0$, $1$, and $2$, along with the sizes of their equivalence classes.
  The figure adopts the stacked format ${\genfrac..{0pt}{1}{n(\sv)}{\sv}}$.}
  \label{figure:Bellnumbers}
\end{figure}

Our next task is to compute the probability that a representative from an equivalance class survives.
We employ the notion of generating functions~\cite{graham1989concrete} to obtain the probability of survival.
For every $j$-pattern sequence $\sv \in \mc{P}_j$, we track the distribution of random variable $T(\sv)$, the number of effective parity-check bits for an element in that class.
This is accomplished by evaluating the probability generating function (PGF) of $T(\sv)$, which takes the form
\begin{equation} \label{generatingFunction}
\Phi_{\sv}(x) = \mathbb{E} \left[ x^{T(\sv)} \right]
% = \sum_{t=0}^{\sum_{q=1}^{j-1}l_q} \Pr (T(\sv)=t)x^t
= \sum_{t=0}^{l_1 + \cdots + l_{j-1}} \Pr (T(\sv)=t)x^t .
\end{equation}
Above, $\Pr (T(\sv)=t)$ is the probability that $t$ parity bits are statistically discriminating, for $j$-pattern sequence $\sv$.
The probability that a particular index sequence with representative class $\sv$ survives at the end of the decoding process is then given by $\Phi_{\sv}(0.5)$.

For example, the $3$-pattern sequence $(1,1,1)$ has generating function $\Phi_{(1,1,1)}(x)=1$ because it corresponds to a valid path in the tree.
The parity bits for a valid sequence match the information bits by construction and, as such, this sequence invariably appears on the output list.
The $3$-pattern sequence $(1,1,3)$ represents states of the form $\{ (i_0, i_1, i_2): i_0=i_1, i_1 \neq i_2 \}$.
From our previous discussion on fragmented codewords, we gather that the first $l_1$ parity bits in this candidate codeword are non-discriminating because the information bits for the first two fragments are drawn from a same message.
On the other hand, the $l_2$ parity check bits in the second sub-block only become non-discriminating when $\wv_{i_0}(0) = \wv_{i_2}(0)$ and $\wv_{i_0}(1) = \wv_{i_2}(1)$.
This conjunction of these events occurs with a probability $\frac{1}{2^{m_0+m_1}}$.
Altogether, the generating function for this 3-pattern sequence is given by $\Phi_{(1,1,3)}(x) = \left( 1 - \frac{1}{2^{m_0+m_1}} \right) x^{l_2} + \frac{1}{2^{m_0+m_1}}$.
It can be verified in an analogous fashion that $\Phi_{(1,2,2)}(x)= \left( 1-\frac{1}{2^{m_0}} \right) x^{l_1+l_2} + \frac{1}{2^{m_0}}$.

Collecting the notions introduced thus far, we can define an aggregate generating function $\boldsymbol{\Phi}(x)$ for the single rooted tree,
\begin{equation} \label{equation:TreeGeneratingFunction}
\boldsymbol{\Phi}(x) = \sum_{\sv \in \mathcal{P}_j} n(\sv) \Phi_{\sv}(x) .
\end{equation}
The expected number of surviving paths within the tree is then given by $\boldsymbol{\Phi}(0.5)$.
In the remainder of this section, we describe the computation of the generating functions for a given $j$-pattern sequence, $\Phi_{\sv}(x)$.
It is pertinent to note that $\Phi_{\sv}(x)$ is sparse;
the coefficient of $x^t$ can only be non-zero when
\begin{equation*}
t \in \left\{ \sum_{q \in S} l_q : \mathcal{S} \subseteq [1:j-1] \right\} . 
\end{equation*}
Thus, it suffices to compute $\Pr (T(\sv)=t)$ for values of $t$ within this set.
We also point out that multiple subsets of $[1:j-1]$ can contribute to a same coefficient.
In other words, there can be distinct subsets, say $\mathcal{S}$ and $\mathcal{S}'$, such that $\sum_{q \in \mathcal{S}} l_q = \sum_{q \in \mathcal{S}'}l_q$.
Altogether, the computation of $\Phi_{\sv}(x)$ mandates inspecting the contribution of all $2^{j-1}$ subsets of $[1:j-1]$. 


\subsection{Statistically Discriminating Parity Bits}
\label{subsection:StatisticallyDiscriminatingParityBits}

Again, consider $j$-pattern sequence $\sv$.
We are interested in events where the parity bits associated with column groups in $G$ are statistically discriminating.
Recall that the $l_q$ parity-check bits in $\pv(q)$ are generated via column group
\begin{equation*}
\begin{bmatrix} G_{0,q-1} \\ \vdots \\ G_{q-1, q-1} \\ \mathbf{0} \end{bmatrix} ,
\end{equation*}
and they become collectively discriminating if and only if at least one entry in
\begin{equation*}
% \left( \wv_{i_0}(0) + \wv_{i_{q}}(0), \ldots, \wv_{i_{q-1}}(q-1) + \wv_{i_q}(q-1), \underline{0} \right)
\left( \wv_{\sv(0)}(0) + \wv_{\sv(q)}(0), \ldots, \wv_{\sv(q-1)}(q-1) + \wv_{\sv(q)}(q-1), \underline{0} \right)
\end{equation*}
is non-zero.
Define $\mathcal{E}_{\sv,\mathcal{S}}$ to be the event where the parity bits $\pv(q)$ with $q \in \mathcal{S}$ are statistically discriminating, but those with indices in $\mathcal{S}^{\mathrm{c}} = [1:n-1] \setminus \mathcal{S}$ are not.
This somewhat intricate concept warrants an example.
Suppose $\mathcal{S} = \{ 1, 3, 5 \}$; then $\mathcal{E}_{\sv,\mathcal{S}}$ is the event where the parity-check bits $\pv(1)$, $\pv(3)$, and $\pv(5)$ essentially become strings of random Bernoulli trials under the randomness in $G$, which must meet prescribed parity requirements for the candidate message to survive.
Whereas the parity constraints for sub-blocks $[1:n-1] \setminus \{ 1, 3, 5 \}$ are fulfilled solely based on the $j$-pattern and/or message fragments matching one another, regardless of the realization of matrix $G$.
Then, taking into account all the possible subsets of $[1:n-1]$, we can rewrite \eqref{generatingFunction} as
\begin{equation} \label{equation:TreeGeneratingFunctionSingleSet}
\Phi_{\sv}(x) = \sum_{\mathcal{S} \subseteq [1:n-1]}
\Pr \left( \mathcal{E}_{\sv,\mathcal{S}}\right) x^{\sum_{q \in \mathcal{S}}l_q} .
\end{equation}
This expression invites a closer look at the summand $\Pr \left( \mathcal{E}_{\sv, \mathcal{S}} \right)$, which can be computed for every $\mathcal{S} \subseteq [1:n-1]$ based on the randomness in the message sequences. 
 
To better understand such events, we further decompose $\mathcal{E}_{\sv, \mathcal{S}}$ into events that occur within specific blocks.
Let $\mathcal{A}_{q,\sv}$ be the event in which parity-check bits of sub-block $q$ are non-discriminating for the $j$-pattern sequence $\sv$.
Based on our previous discussion on fragmented codewords, we have
\begin{equation} \label{equation:GroupNonDiscriminating}
\mathcal{A}_{q,\sv}
= \bigcap_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} \left\{ \wv_{\sv(q)}(j)=\wv_{\sv(j)}(j) \right\} .
\end{equation}
Then, event $\mathcal{E}_{\sv,\mathcal{S}}$ can be expressed as
\begin{equation} \label{EsS}
\mathcal{E}_{\sv,\mathcal{S}}
= \left( \bigcap_{q \in \mathcal{S}^{\mathrm{c}}} \mathcal{A}_{q,\sv} \right)
\bigcap \left( \bigcap_{q \in \mathcal{S}} \mathcal{A}^{\mathrm{c}}_{q,\sv} \right) .
\end{equation}
We emphasize that the analysis of $\Pr \left( \mathcal{E}_{\sv,\mathcal{S}} \right)$ is cumbersome because the events $\mathcal{A}_{q,\sv}$, $q \in [1:j-1]$ are not independent from each other.
Dependencies arise because of re-entries to previously visited levels, as captured by the $j$-pattern sequence $\sv$.
Nevertheless, before moving forward, it is meaningful to characterize the probability of building-block event $\mathcal{A}_{q,\sv}$.

\begin{lemma} \label{P}
Let $j$-pattern sequence $\sv$ be fixed.
The probability that the parity bits of sub-block $\pv(q)$ are non-discriminating is
\begin{equation*}
\Pr \left( \mathcal{A}_{q,\sv}\right) = g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}}m_{j} \right) ,
\end{equation*}
where $g(t)=2^{-t}$.
\end{lemma}
\begin{IEEEproof}
We already know that, based on equivalence class $\sv$, the contribution of block $G_{j,q-1}$ is lost at every location where $\sv(j) = \sv(q)$.
As such, event $\mathcal{A}_{q,\sv}$ corresponds to a situation where candidate message sequence $(\wv_{\sv(0)}(0), \ldots \wv_{\sv(q-1)}(q-1))$ also matches valid partial message $(\wv_{\sv(q)}(0), \ldots \wv_{\sv(q)}(q-1))$ at every locations where $\sv(j) \neq \sv(q)$.
This renders the parity-check bits in $\pv(q)$ non-discriminating.
The probability of this event occurring, conditioned on $\sv$, is given by
\begin{equation}
\begin{split}
\Pr \left( \mathcal{A}_{q,\sv} \right)
&= \Pr \left(\bigcap_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} \left\{ \wv_{\sv(q)}(j)=\wv_{\sv(j)}(j) \right\} \right) \\
&= \prod_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} \Pr \left( \wv_{\sv(q)}(j)=\wv_{\sv(j)}(j) \right) \\
&= \prod_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}}g{(m_{j})}
= g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}}m_{j} \right) ,
\end{split}
\end{equation}
where the second equality is justified through the independence of information bits across distinct messages.
\end{IEEEproof}
%The probability $P\left( \mathcal{A}^e_{q,\sv}\right)$ can be computed as $P\left( \mathcal{A}^e_{q,\sv}\right)=1-P\left( \mathcal{A}^i_{q,\sv}\right)$.

In essence, Lemma~\ref{P} reveals how the equivalence class $\sv$ and the randomness in information bits across messages determine the discriminatory power of $\pv(q)$.
Ultimately, the ability to detect an erroneous codeword through $\pv(q)$ also depends on the randomness in $G$.
Under the right conditions, there is a block activation of the $l_q$ bits; otherwise, they collectively become non-discriminatory.
At this point, we turn to the challenge of computing the joint probability that parity-check bits across blocks are discriminating.
To account for dependencies among column groups, we express $\Pr \left(\mathcal{E}_{\sv,\mathcal{S}}\right)$ using conditional probability,
\begin{equation} \label{PEsS}
\Pr \left(\mathcal{E}_{\sv,\mathcal{S}}\right)
= \Pr \left( \bigcap_{q \in \mathcal{S}}\mathcal{A}^{\mathrm{c}}_{q,\sv} \Bigg| \bigcap_{q \in \mathcal{S}^{\mathrm{c}}}\mathcal{A}_{q,\sv} \right)
\Pr \left( \bigcap_{q \in \mathcal{S}^{\mathrm{c}}}\mathcal{A}_{q,\sv} \right) .
\end{equation}

We begin our treatment of \eqref{PEsS} by examining the rightmost term.
We can apply the chain rule of probability to this expression, which yields
\begin{equation} \label{equation:ConditionalChainRule}
\Pr \left( \bigcap_{q \in \mathcal{S}^{\mathrm{c}}} \mathcal{A}_{q,\sv} \right)
= \prod_{q \in \mathcal{S}^{\mathrm{c}}} \Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \mathcal{S}^{\mathrm{c}} \cap [1:q-1]}\mathcal{A}_{\ell, \sv}\right) .
\end{equation}
Inspecting \eqref{equation:GroupNonDiscriminating}, we gather that events of the form $\mathcal{A}_{q,\sv}$ are subject to a partial order through set inclusion.
In particular, suppose that $\sv(q) = \sv(\ell)$ with $\ell < q$, then $\mathcal{A}_{q,\sv} \subset \mathcal{A}_{\ell,\sv}$.
This property immediately implies that the most constraining condition within this branch of the partial order is $\mathcal{A}_{p,\sv}$ where $p = \max \left\{ \ell \in [1 : q-1] | \sv(q) = \sv(\ell) \right\}$.
On the other hand, when $\sv(q) \neq \sv(\ell)$, the events $\mathcal{A}_{q,\sv}$ and $\mathcal{A}_{\ell,\sv}$ are independent.
This follows from the fact that, in this latter case, the conditions in \eqref{equation:GroupNonDiscriminating} operate on different pairs of fragments altogether.
The fact that information bits are selected independently across messages is therefore enough to ensure independence.
While the situation is slightly more involved when accounting for $\mathcal{S}$, the concepts are essentially identical.
These observations invite the following definitions,
\begin{align}
\underline{\mathcal{G}}_{q,\mathcal{S},\sv} &= [1:q-1] \cap \mathcal{S}^{\mathrm{c}} \cap \{k \in [1:j-1]: \sv(k) \neq \sv(q)\} 
\label{equation:Gunderline} \\
\underline{\mathcal{Q}}_{q,\mathcal{S},\sv} &= [1:q-1] \cap \mathcal{S}^{\mathrm{c}} \cap \{k \in [1:j-1]: \sv(k) = \sv(q)\} .
\label{equation:Qunderline}
\end{align}
In words, $\underline{\mathcal{G}}_{q,\mathcal{S},\sv}$ contains the numbers of the sub-blocks that precede sub-block $q$ (excluding sub-block $0$), feature a different level than $\sv(q)$, and are not included in $\mathcal{S}$.
Likewise, $\underline{\mathcal{Q}}_{q,\mathcal{S},\sv}$ contains the numbers of the sub-blocks that precede sub-block $q$ (excluding sub-block $0$), possess the same level as $\sv(q)$, and are not included in $\mathcal{S}$.
Based on this notation, we formalize the above discussion into a lemma.

\begin{lemma} \label{P1}
Consider equivalence class $\sv$ and set $\mathcal{S} \subset [1:n-1]$.
Then, when the conditional event has positive probability, we get
\begin{equation} \label{equation:P1}
\Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \mathcal{S}^{\mathrm{c}} \cap [1:q-1]}\mathcal{A}_{\ell, \sv}\right)
%\Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv} \right)
= g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} m_{j}
- \sum_{\substack{k \in [0:p-1] \\ \sv(p) \neq \sv(k)}} m_{k} \right),
\end{equation}
where
$p = \max \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}$ and $g(t)=2^{-t}$.
\end{lemma}
\begin{IEEEproof}
Taking into consideration the independence structure identified above, we immediately get
\begin{equation} \label{equation:P1reduced}
\begin{split}
\Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \mathcal{S}^{\mathrm{c}} \cap [1:q-1]}\mathcal{A}_{\ell, \sv}\right)
&= \Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell, \sv} ,
\bigcap_{\ell \in \underline{\mathcal{G}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell, \sv} \right) \\
&= \Pr \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell, \sv} \right) .
% = \Pr \left( \mathcal{A}_{q,\sv} \Bigg| \mathcal{A}_{p,\sv} \right)
\end{split}
\end{equation}
We know that events of the form $\mathcal{A}_{q,\sv}$ form a partial order through set inclusion.
Moreover, $\mathcal{A}_{k,\sv} \subset \mathcal{A}_{j,\sv}$ whenever j < k and $\sv(j) = \sv(k)$.
This leads to the following two equalities:
\begin{equation*}
\bigcap_{k \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{k,\sv} = \mathcal{A}_{p, \sv}
\end{equation*}
and $\mathcal{A}_{q,\sv} \cap \mathcal{A}_{p, \sv} = \mathcal{A}_{q,\sv}$, where $p = \max \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}$.
Substituting these expressions into the conditional probability of \eqref{equation:P1reduced}, we get
\begin{equation} \label{equation:P1proof}
\begin{split}
\Pr & \left( \mathcal{A}_{q,\sv} \Bigg| \bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv}\right)
= \Pr \left( \mathcal{A}_{q,\sv} \Bigg| \mathcal{A}_{p,\sv} \right) \\
&= \frac{ \Pr \left( \mathcal{A}_{q,\sv} \bigcap \mathcal{A}_{p,\sv} \right) }
{\Pr \left( \mathcal{A}_{p,\sv} \right)}
= \frac{ \Pr \left( \mathcal{A}_{q,\sv} \right) } {\Pr \left(\mathcal{A}_{p,\sv} \right)} \\
&= g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} m_{j}
- \sum_{\substack{k \in [0:p-1] \\ \sv(p) \neq \sv(k)}} m_{k} \right) .
\end{split}
\end{equation}
The fourth inequality in \eqref{equation:P1proof} is obtained by applying Lemma~\ref{P} and using straightforward properties of the function $g(t) = 2^{-t}$.
\end{IEEEproof}

Together Lemma~\ref{P1} and \eqref{equation:ConditionalChainRule} offer a means to compute the rightmost term in \eqref{PEsS}.
We then turn to the leftmost term on the right-hand-side of \eqref{PEsS}.
To facilitate the description of this slightly more involved expression, we need to expand special cases beyond \eqref{equation:Gunderline} and \eqref{equation:Qunderline}.
Specifically, for every $q \in [1:n-1]$, we introduce the following additional cases:
\begin{align*}
\overline{\mathcal{G}}_{q,\mathcal{S},\sv} &= [q+1:n-1] \cap \mathcal{S}^{\mathrm{c}}\cap \{k \in [1:n-1]:\sv(k) \neq \sv(q)\} \\
\overline{\mathcal{Q}}_{q,\mathcal{S},\sv} &= [q+1:n-1] \cap \mathcal{S}^{\mathrm{c}} \cap \{k \in [1:n-1]:\sv(k) = \sv(q)\} \\
\underline{\tilde{\mathcal{G}}}_{q,\mathcal{S},\sv} &= [1:q-1] \cap \mathcal{S} \cap \{k \in [1:n-1]: \sv(k) \neq \sv(q)\} \\
\underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} &= [1:q-1] \cap \mathcal{S} \cap \{k \in [1:n-1]: \sv(k) = \sv(q)\}.
\end{align*}
Above, $\underline{\tilde{\mathcal{G}}}_{q,\mathcal{S},\sv}$ contains the numbers of the sub-blocks that trail sub-block $q$, feature a different level than $\sv(q)$, and are not included in $\mathcal{S}$.
The set $\underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}$ contains the numbers of the sub-blocks that trail sub-block $q$, possess the same level as $\sv(q)$, and are not included in $\mathcal{S}$.
The last two conditions, $\underline{\tilde{\mathcal{G}}}_{q,\mathcal{S},\sv}$ and $\underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}$ are analogous to $\underline{\mathcal{G}}_{q,\mathcal{S},\sv}$ and $\underline{\mathcal{Q}}_{q,\mathcal{S},\sv}$, albeit they contain numbers belonging to $\mathcal{S}$ rather than its complement.

The strategy to tackle
\begin{equation} \label{equation:ConditonalProb}
\Pr \left( \bigcap_{q \in \mathcal{S}} \mathcal{A}^{\mathrm{c}}_{q,\sv} \Bigg| \bigcap_{\ell \in \mathcal{S}^{\mathrm{c}}} \mathcal{A}_{\ell,\sv} \right)
\end{equation}
is similar to our previous step.
We apply the chain rule of probability and analyze the relation between events.
The expanded version of \eqref{equation:ConditonalProb} can be written as
\begin{equation} \label{equation:ConditonalProbChainRule}
\prod_{q \in \mathcal{S}} \Pr \left( \mathcal{A}^{\mathrm{c}}_{q,\sv} \Bigg| \bigcap_{\ell \in \mathcal{S}^{\mathrm{c}}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \mathcal{S} \cap [1:q-1]} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) .
\end{equation}
We can further partition the conditional events via
\begin{gather}
\mathcal{S}^{\mathrm{c}} = \underline{\mathcal{G}}_{q,\mathcal{S},\sv} \uplus \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}
\uplus \overline{\mathcal{G}}_{q,\mathcal{S},\sv} \uplus \overline{\mathcal{Q}}_{q,\mathcal{S},\sv} \\
\mathcal{S} \cap [1:q-1] = \underline{\tilde{\mathcal{G}}}_{q,\mathcal{S},\sv} \uplus \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} .
\end{gather}
The event $\mathcal{A}^{\mathrm{c}}_{q,\sv}$ in which parity-check bits of sub-block $q$ are discriminating; together with what occurs at level $\sv(q)$, namely $\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv} \uplus \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv}$ and $\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv}$, is independent of sub-blocks associated with other levels, namely $\bigcap_{\ell \in \underline{\mathcal{G}}_{q,\mathcal{S},\sv} \uplus \overline{\mathcal{G}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv}$ and $\bigcap_{k \in \underline{\tilde{\mathcal{G}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv}$.
As before, this property follows from the fact that, at levels other than $\sv(q)$, the conditions in \eqref{equation:GroupNonDiscriminating} operate on different pairs of fragments altogether.
Since information bits are selected independently across messages, this is enough to ensure independence between the groupings above.
Thus, \eqref{equation:ConditonalProbChainRule} reduces to
\begin{equation} \label{equation:ReducedConditonalProbChainRule}
\begin{split}
&\prod_{q \in \mathcal{S}} \Pr \left( \mathcal{A}^{\mathrm{c}}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) \\
&= \prod_{q \in \mathcal{S}} \left( 1 - \Pr \left( \mathcal{A}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) \right) .
\end{split}
\end{equation}
The probability expression in \eqref{equation:ReducedConditonalProbChainRule} is in a form reminiscent of Lemma~\ref{P1}.
At this stage, we proceed by breaking the conditional expression above into special cases.

\paragraph{Case I -- $( \overline{\mathcal{Q}}_{q,\mathcal{S},\sv} \neq \emptyset )$}
If this set is not empty, then there exists an element $\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}$, $\ell > q$, such that the parity bits generated by column group~$\ell$ are non-discriminating.
This implies that vector $( \wv_{\sv(0)}(0) + \wv_{\sv(\ell)}(0), \ldots, \wv_{\sv(\ell-1)}(\ell-1) + \wv_{\sv(\ell)}(\ell-1)) = \underline{0}$.
Since $\sv(\ell) = \sv(q)$, we deduce that sub-vector $( \wv_{\sv(0)}(0) + \wv_{\sv(q)}(0), \ldots, \wv_{\sv(q-1)}(q-1) + \wv_{\sv(q)}(q-1)) = \underline{0}$.
Thus, the parity-check bits generated by column group~$q$ are non-discriminating and
\begin{equation} \label{caseI}
\Pr \left( \mathcal{A}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) = 1 .
\end{equation}

\paragraph{Case II -- $( \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} \neq \emptyset )$}
If this set in not empty, then there exists an element $k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}$, $k < q$, such that the parity bits generated by column group~$k$ are discriminating.
In other words, vector $( \wv_{\sv(0)}(0) + \wv_{\sv(k)}(0), \ldots, \wv_{\sv(k-1)}(k-1) + \wv_{\sv(k)}(k-1) )$ is non-zero.
Yet, this vector appears as a sub-component of $( \wv_{\sv(0)}(0) + \wv_{\sv(q)}(0), \ldots, \wv_{\sv(q-1)}(q-1) + \wv_{\sv(q)}(q-1))$ and, consequently, the latter vector must also be a non-zero vector.
By Lemma~\ref{lemma:RandomGenerator}, this implies that the parity-check bits associated with column group~$q$ are discriminatory and
\begin{equation} \label{caseII}
\Pr \left( \mathcal{A}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) = 0 .
\end{equation}

\paragraph{Case III -- $( \overline{\mathcal{Q}}_{q,\mathcal{S},\sv} = \emptyset$ and $\underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} = \emptyset )$}
In this case, we get
\begin{equation} \label{caseIII}
\begin{split}
\Pr & \left( \mathcal{A}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{\ell \in \overline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv},
\bigcap_{k \in \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv}} \mathcal{A}^{\mathrm{c}}_{k,\sv} \right) \\
&= \Pr \left( \mathcal{A}_{q,\sv} \Bigg|
\bigcap_{\ell \in \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}} \mathcal{A}_{\ell,\sv} \right)
\end{split}
\end{equation}
and we can apply Lemma~\ref{P1}, which gives us a means to compute the desired probability.

\begin{remark}
The fourth case where both $\overline{\mathcal{Q}}_{q,\mathcal{S},\sv} \neq \emptyset$ and $\underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} \neq \emptyset$ cannot occur and need not be considered.
The first condition prevents $\pv(q)$ from being statistically discriminating, whereas the second condition forces these parity-check bits to be discriminating.
In such scenarios, $\Pr \left( \mathcal{E}_{\sv,\mathcal{S}} \right)$ does not admit the conditional form of \eqref{PEsS}, but it can readily be identified as having probability zero.
\end{remark}

We collect the results discussed above and summarize our findings in the form of a proposition.

\begin{proposition} \label{proposition:ProbabilityPatternBasedEvent}
Consider equivalence class $\sv$ and set $\mathcal{S} \subset [1:n-1]$.
The probability that the parity-check bits $\pv(q)$ with $q \in \mathcal{S}$ are statistically discriminating, and those with indices in $\mathcal{S}^{\mathrm{c}} = [1:n-1] \setminus \mathcal{S}$ are non-discriminating is given by
\begin{equation}
\begin{split}
\Pr \left( \mathcal{E}_{\sv,\mathcal{S}} \right)
&= \prod_{q \in \mathcal{S}^{\mathrm{c}}} g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} m_{j}
- \sum_{\substack{k \in [0:p-1] \\ \sv(p) \neq \sv(k)}} m_{k} \right) \\
&\times \prod_{q \in \mathcal{S}} \left[ 1 - \left[
\mathbbm{1}_{ \left\{ \overline{\mathcal{Q}}_{q,\mathcal{S},\sv} \neq \emptyset \right\} }
+ \mathbbm{1}_{ \left\{ \overline{\mathcal{Q}}_{q,\mathcal{S},\sv} = \emptyset \right\} }
\mathbbm{1}_{ \left\{ \underline{\tilde{\mathcal{Q}}}_{q,\mathcal{S},\sv} = \emptyset \right\} }
g \left( \sum_{\substack{j \in [0:q-1] \\ \sv(q) \neq \sv(j)}} m_{j}
- \sum_{\substack{k \in [0:p-1] \\ \sv(p) \neq \sv(k)}} m_{k} \right)
\right] \right]
\end{split}
\end{equation}
where $\mathbbm{1}_{ \{ \cdot \} }$ is the set indicator function, $p = \max \underline{\mathcal{Q}}_{q,\mathcal{S},\sv}$ and $g(t)=2^{-t}$.
\end{proposition}

This proposition, together with \eqref{equation:TreeGeneratingFunction} and \eqref{equation:TreeGeneratingFunctionSingleSet}, provides an algorithmic procedure to compute the expected number of erroneous paths that survive the decoding process.
While the proposition is stated for the full length of the transmission process, the reader will notice that the result can also be applied at any stage of the decoding process.
Hence, the expected number of erroneous surviving paths at level $j-1$ is given by,
\begin{equation*}
\mathbb{E}[L_{j-1}] = \sum_{\sv \in \mc{P}_j} n(\sv) \Phi_{\sv} \left( \frac{1}{2} \right) - 1,
\quad j \in [1:n].
\end{equation*}

Our expression for the expected number of surviving candidate codewords at the end of the tree decoding process is convoluted.
Unfortunately, there is no apparent structure, beyond the presence of equivalence classes, that enable a reduction in computational complexity.
It is pertinent to mention that the Bell numbers grow rapidly and, as such, the computation of the expected number of surviving paths through the tree can be challenging.
Nevertheless,  exact numbers can be obtained for the parameters we are interested in.






% The generating function can be efficiently computed by leveraging the Markov structure of the pattern sequences. Specifically, $\Phi_{\sv}(x)$ can be factorized as,
% \begin{align*}
% \Phi_{\sv}(x) = \psi_{\sv}(x)\Phi_{\sv(1:j-1)}(x),
% \end{align*}
% where $\psi_{\sv}(x)$ tracks the probability that $l_{j-1}$ parity-check bits, that correspond to the $j^{\mathrm{th}}$ sub-block are effective for the pattern sequence $\sv$. This function takes the form,
% \begin{align*}
% \psi_{\sv}(x) = c(\sv)x^{l_{j-1}}+1-c(\sv),
% \end{align*}
% where $c(\sv)$ denotes the probability that $l_{j-1}$ parity-check bits at stage $j-1$ are effective for the states represented by the sequence $\sv$. Based on our previous discussion on fragmented codewords, the quantity $c(\sv)$ can be evaluated using \eqref{ljtakeeffect} as,
% \begin{align*}
% c(\sv) = 1-\prod_{\substack{q=1 \\ \sv(q) \neq \sv(j)}}^{j-1} 2^{-m_q}.
% \end{align*}
% In this manner, the generating function $\Phi_{\sv}(x)$ of the pattern sequence $\sv$ can be computed recursively, using the generating function of $\sv(1:j-1)$ and the initial condition $\Phi_{\sv(1)}(x)=1$. It is easy to see that a path represented by the $j$-pattern sequence $\sv$ survives the stage $j$ of decoding process with a probabilities given by $\Phi_{\sv}\left(\frac{1}{2}\right)$. Finally, the expected number of erroneous surviving paths at level $j$ can be computed as,
% \begin{align*}
% \mathbb{E}[L_j] = \sum_{\sv \in \mc{P}_j}n(\sv)\Phi_{\sv}\left(\frac{1}{2}\right)-1,
% \end{align*}
% where $n(\sv)$ can be computed using Lemma \ref{Number of states}.

%Though this procedure gives a way to compute the expected number of erroneous paths numerically, it mandates keeping track of generating functions for all the $j$-pattern sequences at stage $j$. As mentioned earlier, this number grows exponentially with $j$ and can only be done for a modest number of sub-blocks. However, a close upper bound on the expected number of erroneous paths can be obtained with much fewer computations, if there is a significant stretch of sub-blocks in the initial phases of the tree with the same number of information bits ( or parity-check bits). However, it must be noted that this approach does not provide an exact formulation for the expected number of erroneous paths, since the first sub-block contains only information bits and no parity-check bits. However, the discrepancy arises only because of the assumption that the first sub-block exhibits the same structure as the subsequent few sub-blocks and this difference is negligible for all practical purposes. 


